Scaling Transformer-Based Novel View Synthesis Models with Token Disentanglement and Synthetic Data

Large transformer-based models have made significant progress in generalizable novel view synthesis (NVS) from sparse input views, generating novel viewpoints without the need for test-time optimization. However, these models are constrained by the limited diversity of publicly available scene datasets, making most real-world (in-the-wild) scenes out-of-distribution. To overcome this, we incorporate synthetic training data generated from diffusion models, which improves generalization across unseen domains. While synthetic data offers scalability, we identify artifacts introduced during data generation as a key bottleneck affecting reconstruction quality. To address this, we propose a token disentanglement process within the transformer architecture, enhancing feature separation and ensuring more effective learning. This refinement not only improves reconstruction quality over standard transformers but also enables scalable training with synthetic data. As a result, our method outperforms existing models on both in-dataset and cross-dataset evaluations, achieving state-of-the-art results across multiple benchmarks while significantly reducing computational costs. Project page: https://scaling3dnvs.github.io/

==> metrics/cross_Resolution_generalization.tex <==







\definecolor{lightyellow}{rgb}{1,1, 0.8}
\definecolor{yellow}{rgb}{1,0.97, 0.65}
\definecolor{orange}{rgb}{1, 0.85, 0.7}
\definecolor{tablered}{rgb}{1, 0.7, 0.7}


\begin{table}[t!]
\caption{\textbf{Quantitative comparisons for scaling up  across different datasets for a resolution of 256 with a batch size of 64
} }
\vspace{-0.1in}
% \begin{minipage}{\textwidth}
% \resizebox{0.99\linewidth}{!}{
% \begin{tabular}{r|ccc|ccc } 
%     \midrule
%     LGM~\citep{tang2024lgm} (Res-256) & 20.79 & 0.813  & 0.158 & 21.44  & 0.832 & 0.122 \\
%     GS-LRM~\citep{zhang2024gslrmlargereconstructionmodel} (Res-256) &   28.98  &  \cellcolor{orange}0.926 &  0.074  &  \cellcolor{orange}29.59 &  \cellcolor{orange}0.944 &  0.051 \\
    
%      LVSM (Res-256)  & 32.47  &   0.944 &  0.037 &  31.71 &  0.957 &  0.027  \\
% \end{tabular}
% }
% \label{tab:compare_objects}
% \hfill
% \end{minipage}%

\resizebox{0.99\linewidth}{!}{
\begin{tabular}{r|ccc|ccc} 
    Method&\multicolumn{3}{c}{Test-resolution 256$\times$256}&  \multicolumn{3}{c}{Test-resolution 256$\times$448}  \\ 
     & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\) & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\)  \\ 
    \midrule 
            \multicolumn{7}{c}{DL3DV Dataset}  \\
    \midrule 

     LVSM & 28.89 & 0.894 & 0.108 &  27.45 & 0.880  &0.078  \\

     Ours&  30.02 & 0.918  & 0.058    & 28.17 & 0.890   &0.071   \\
           \multicolumn{7}{c}{Re10K Dataset}  \\
    \midrule 

     LVSM & 28.89 & 0.894 & 0.108 & 27.45 & 0.880  &0.078  \\

     Ours&  TBD & TBD  & TBD    & 28.17 & 0.8899   &0.0706   \\

\end{tabular}
}
\label{tab:ablation}
\vspace{0.05in}
\end{table}










==> metrics/cross_dataset.tex <==
\definecolor{lightyellow}{rgb}{1,1, 0.8}
\definecolor{yellow}{rgb}{1,0.97, 0.65}
\definecolor{orange}{rgb}{1, 0.85, 0.7}
\definecolor{tablered}{rgb}{1, 0.7, 0.7}


\begin{table*}[t!]
\caption{\textbf{Quantitative comparisons on scene level synthesis across different datasets for a resolution of 256 with a batch size of 64 
} }
\vspace{-0.1in}
% \begin{minipage}{\textwidth}
% \resizebox{0.99\linewidth}{!}{
% \begin{tabular}{r|ccc|ccc } 
%     \midrule
%     LGM~\citep{tang2024lgm} (Res-256) & 20.79 & 0.813  & 0.158 & 21.44  & 0.832 & 0.122 \\
%     GS-LRM~\citep{zhang2024gslrmlargereconstructionmodel} (Res-256) &   28.98  &  \cellcolor{orange}0.926 &  0.074  &  \cellcolor{orange}29.59 &  \cellcolor{orange}0.944 &  0.051 \\
    
%      LVSM (Res-256)  & 32.47  &   0.944 &  0.037 &  31.71 &  0.957 &  0.027  \\
% \end{tabular}
% }
% \label{tab:compare_objects}
% \hfill
% \end{minipage}%

\resizebox{0.99\linewidth}{!}{
\begin{tabular}{r|ccc|ccc|ccc} 
    &  \multicolumn{3}{c}{RealEstate10k~\citep{realestate10k_zhou2018stereo}}&  \multicolumn{3}{c}{ACID~\citep{realestate10k_zhou2018stereo}}&  \multicolumn{3}{c}{DL3DV~\citep{realestate10k_zhou2018stereo}}  \\ 
    & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\) & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\) & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\)  \\ 
    \midrule
    pixelSplat~\citep{charatan2024pixelsplat} & 26.09 & 0.863  & 0.136 \\
    MVSplat~\citep{chen2024mvsplatefficient3dgaussian} & 26.39 & 0.869  & 0.128 \\
    GS-LRM~\citep{zhang2024gslrmlargereconstructionmodel} & 28.10 & 0.892  & 0.114 \\
     LVSM & 29.67 & 0.906 & 0.098 \\
     Ours& TODO & TODO &TODO\\
\end{tabular}
}
\label{tab:compare_scenes}
\vspace{0.05in}
\end{table*}










==> metrics/crossdataset_visuals.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}


      \includegraphics[width=1\linewidth, height=\linewidth]{real_results/pose_image_walter.jpg}

      \includegraphics[width=1\linewidth]{real_results/arcde.jpg}


    %   \includegraphics[width=1\linewidth]{/input_new/1035.jpg}
      \caption{TASK-1}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}

      \includegraphics[width=1\linewidth]{real_results/room_depth.jpg}
      \includegraphics[width=1\linewidth,height=1\linewidth]{real_results/car.jpg}

  



    %   \includegraphics[width=1\linewidth]{/spade/1035.jpg}
      \caption{TASK-2}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/12.jpg}
        \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/22.jpg}



      % \includegraphics[width=1\linewidth]{results/seg_hed/spade/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/pix2pixhd/1035.jpg}
      \caption{Multi-T2I Adapter}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}

      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/13.jpg}
      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/23.jpg}



      % \includegraphics[width=1\linewidth]{results/seg_hed/piti/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/inade/1035.jpg}
      \caption{Multi-T2I Adapter}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/12.jpg}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/22.jpg}


      % \includegraphics[width=1\linewidth]{results/seg_hed/adapter/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/ddpm/1035.jpg}
      \caption{Multi-ControlNet}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/13.jpg}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/23.jpg}

      % \includegraphics[width=1\linewidth]{results/seg_hed/control/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/tedigan/1035.jpg}
      \caption{Multi-ControlNet}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}



        \includegraphics[width=1\linewidth]{real_results/ours/pose/855.jpg}


      \includegraphics[width=1\linewidth]{real_results/ours/arc/911.jpg}


      % \includegraphics[width=1\linewidth]{results/seg_hed/ours/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/1035.jpg}
      \caption{OURS}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
        \includegraphics[width=1\linewidth]{real_results/ours/pose/857.jpg}
      \includegraphics[width=1\linewidth]{real_results/ours/arc/892.jpg}
      % \includegraphics[width=1\linewidth]{results/seg_hed/ours/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/1035.jpg}
      \caption{Ours}
    \end{subfigure}
    \vspace{-3mm}    \caption{\textbf{Qualitative comparisons cross dataset evaluations}. Figure illustrates the advantage of utilizing synthetic data. Here we present the results of LVSM and OUR model on an out of distribution dataset DL3DV.}
    \label{fig:cross_datasetvisuals}
    \vspace{-4mm}
  \end{figure*}


==> metrics/metrics_objaverse.tex <==

% \begin{table}[t!]
% \caption{\textbf{Quantitative comparisons on object-level (left) and scene-level (right) view synthesis.}
% For the object-level comparison, we matched the baseline settings with GS-LRM~\citep{zhang2024gslrmlargereconstructionmodel} in both input 
% }
% \vspace{-0.1in}
% % \begin{minipage}{\textwidth}
% \resizebox{0.99\linewidth}{!}{
% \begin{tabular}{r|ccc|ccc } 
%     & \multicolumn{3}{c|} {ABO~\citep{collins2022abodatasetbenchmarksrealworld}} &  \multicolumn{3}{c} {GSO~\citep{downs2022gso}} \\ 
%     & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\) & PSNR \(\uparrow\) & SSIM \(\uparrow\) & LPIPS \(\downarrow\) \\ 
%     \midrule
%     LGM~\citep{tang2024lgm} (Res-256) & 20.79 & 0.813  & 0.158 & 21.44  & 0.832 & 0.122 \\
%     GS-LRM~\citep{zhang2024gslrmlargereconstructionmodel} (Res-256) &   28.98  &  0.926 &  0.074  &  29.59 &  0.944 &  0.051 \\
    
%      LVSM (Res-256)  & 32.47  &   0.944 &  0.037 &  31.71 &  0.957 &  0.027  \\
%     OURS (Res-256)  & 32.47  &   0.944 &  0.037 &  31.71 &  0.957 &  0.027  \\
% \end{tabular}
% }
% % \label{tab:compare_objects}
% % \hfill
% % \end{minipage}%


% \label{tab:compare_scenes}
% \vspace{0.05in}
% \end{table}

\definecolor{lightyellow}{rgb}{1,1, 0.8}
\definecolor{yellow}{rgb}{1,0.97, 0.65}
\definecolor{orange}{rgb}{1, 0.85, 0.7}
\definecolor{tablered}{rgb}{1, 0.7, 0.7}


\begin{table*}[t!]
\caption{\textbf{Quantitative comparisons on scene-level synthesis across different datasets for a resolution of 256 with a batch size of 32.} }
\vspace{-0.1in}
% \begin{minipage}{\textwidth}
% \resizebox{0.99\linewidth}{!}{
% \begin{tabular}{r|ccc|ccc } 
%     \midrule
%     LGM~\citep{tang2024lgm} (Res-256) & 20.79 & 0.813  & 0.158 & 21.44  & 0.832 & 0.122 \\
%     GS-LRM~\citep{zhang2024gslrmlargereconstructionmodel} (Res-256) &   28.98  &  \cellcolor{orange}0.926 &  0.074  &  \cellcolor{orange}29.59 &  \cellcolor{orange}0.944 &  0.051 \\
    
%      LVSM (Res-256)  & 32.47  &   0.944 &  0.037 &  31.71 &  0.957 &  0.027  \\
% \end{tabular}
% }
% \label{tab:compare_objects}
% \hfill
% \end{minipage}%

\resizebox{0.99\linewidth}{!}{
\begin{tabular}{r|ccc|ccc|ccc} 
    &  \multicolumn{3}{c}{GSO~\citep{realestate10k_zhou2018stereo}}&  \multicolumn{3}{c}{ABO~\citep{realestate10k_zhou2018stereo}}&  \multicolumn{3}{c}{DTU~\citep{realestate10k_zhou2018stereo}}  \\ 
    & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\) & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\) & PSNR \(\uparrow\) & SSIM \(\uparrow\)  & LPIPS \(\downarrow\)  \\ 
    \midrule
   LGM~\citep{tang2024lgm} & 26.39 & 0.869  & 0.128& 26.09 & 0.863  & 0.136 &  TBD & TBD  & TBD   \\
    GS-LRM~\citep{zhang2024gslrmlargereconstructionmodel} & 28.10 & 0.892  & 0.114& 26.09 & 0.863  & 0.136 &  TBD & TBD  & TBD   \\
     LVSM & 29.67 & 0.906 & 0.098 & 26.09 & 0.863  & 0.136 &  TBD & TBD  & TBD  \\
     Ours& TBD & TBD &TBD& TBD & TBD &TBD & TBD & TBD &TBD \\
\end{tabular}
}
\label{tab:compare_objects}
\vspace{0.05in}
\end{table*}










==> metrics/visuals.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{real_results/cycle_hed.jpg}


      \includegraphics[width=1\linewidth, height=\linewidth]{real_results/pose_image_walter.jpg}

      \includegraphics[width=1\linewidth]{real_results/arcde.jpg}


    %   \includegraphics[width=1\linewidth]{/input_new/1035.jpg}
      \caption{TASK-1}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{real_results/garden_seg.jpg}

      \includegraphics[width=1\linewidth]{real_results/room_depth.jpg}
      \includegraphics[width=1\linewidth,height=1\linewidth]{real_results/car.jpg}

  



    %   \includegraphics[width=1\linewidth]{/spade/1035.jpg}
      \caption{TASK-2}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/2.jpg}
      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/12.jpg}
        \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/22.jpg}



      % \includegraphics[width=1\linewidth]{results/seg_hed/spade/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/pix2pixhd/1035.jpg}
      \caption{Multi-T2I Adapter}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}

      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/10.jpg}
      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/13.jpg}
      \includegraphics[width=1\linewidth]{real_results/ours/adapter_real_results/23.jpg}



      % \includegraphics[width=1\linewidth]{results/seg_hed/piti/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/inade/1035.jpg}
      \caption{Multi-T2I Adapter}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/3.jpg}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/12.jpg}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/22.jpg}


      % \includegraphics[width=1\linewidth]{results/seg_hed/adapter/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/ddpm/1035.jpg}
      \caption{Multi-ControlNet}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/2.jpg}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/13.jpg}
       \includegraphics[width=1\linewidth]{real_results/ours/control_real_Results/23.jpg}

      % \includegraphics[width=1\linewidth]{results/seg_hed/control/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/tedigan/1035.jpg}
      \caption{Multi-ControlNet}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}


      \includegraphics[width=1\linewidth]{real_results/ours/garden/868.jpg}

        \includegraphics[width=1\linewidth]{real_results/ours/pose/855.jpg}


      \includegraphics[width=1\linewidth]{real_results/ours/arc/911.jpg}


      % \includegraphics[width=1\linewidth]{results/seg_hed/ours/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/1035.jpg}
      \caption{OURS}
    \end{subfigure}
    \begin{subfigure}[t]{0.115\linewidth}
      \captionsetup{justification=centering, labelformat=empty, font=scriptsize}
      \includegraphics[width=1\linewidth]{real_results/ours/garden/869.jpg}
        \includegraphics[width=1\linewidth]{real_results/ours/pose/857.jpg}
      \includegraphics[width=1\linewidth]{real_results/ours/arc/892.jpg}
      % \includegraphics[width=1\linewidth]{results/seg_hed/ours/000000019221.jpg}
    %   \includegraphics[width=1\linewidth]{/1035.jpg}
      \caption{Ours}
    \end{subfigure}
    \vspace{-3mm}   \caption{\textbf{Qualitative comparisons In-distribution evaluations}. We present the results produced by different methods and their  Here we present the results of LVSM and OUR model on an out of distribution dataset DL3DV.}
    \label{fig:visuals}
    \vspace{-4mm}
  \end{figure*}


==> sec/cooments.tex <==
% Generalizable novel view synthesis (NVS) from sparse inputs has been influenced by a recent trend where a pure transformer based method is trained with large amounts of 3D data. Such kind of synthesis enables to perform fast real time synthesis of novel view with a pure feed forward models. Recent works have shown improvement of about $1.5-2 dB$ on existing datasets by eliminating  3D inductive biases and a pure decoder based transformer model. However the efficiency and scalability of such models from data perspective and model perspective is yet to be studied in a detailed manner. In this work we take a look at the role of model architecture, 3D informed features and the relevance of data on the generalizability of novel view synthesis models. Our major contribution is two fold -- we build upon the deficits of previous methods and present a novel transformer block design that substantially improves the efficiency of transformer based NVS models. We also overcome the data limitation in 3D reconstruction by developing a pipeline that can effectively leverage synthetic data for improve the reconstruction quality on out of distribution datasets.  Through the combination of these design choices, we achieve state of the art results on various benchmarks for in-dataset and cross-dataset performance for the task of NVS utilizing substantially lower computational resources.

% \SKC{
% Maybe something like --



% In addition, the training and inference for our method is substantially more efficient in both memory and runtime-performance.
% }

% As our base framework for the cross-domain generalizable NVS model, we adopt the Large View Synthesis Model (LVSM). LVSM employs a transformer network to synthesize a target view from two or more source views, along with their camera poses and the target camera pose. We selected LVSM because its simple transformer-based architecture achieves state-of-the-art reconstruction quality for 3D NVS across multiple benchmarks. Upon closer examination, however, we identified key limitations that could hinder model scalability. LVSM struggles when information required for the target view appears in only one of the source views, leading to failure cases (Figure 1). Additionally, we observed texture sticking, where details from a source view persist in the synthesized target view even when they should not be present.  We also examine LVSM’s efficiency and find that its architecture introduces unnecessary computational overhead. In principle, all transformer layers should be optimized for target view reconstruction since only the target features contribute to the loss function, even though both the source and target features pass through the same transformer block. However, due to the design of the basic transformer block, some of the layers in LVSM retain unused source features, diverting some of its modeling capacity away from the target view [Insert figure reference]. This issue arises because the transformer blocks do not explicitly distinguish between source and target tokens, causing source features to be entangled with target features throughout all layers instead of being separately processed. These inefficiencies highlight areas where LVSM needs improvement to effectively scale up NVS.



% where PCA projections across transformer layers demonstrate that our network more effectively utilizes transformer capacity, prioritizing accurate target view synthesis while efficiently processing source information.







% Neural network based Scene representation has seen some substantial progress over the past couple of years. Neural radiance fields paved the way towards optimizing scenes using sparse views sampled from the scene and produced excellent results compared to traditional graphics based methods. NERFs were specifically designed for a case by case basis where a new NERF needs to be trained for each scene. Moreover optimizing and rendering from NERFs takes a couple of hours to minutes for recent works. Recently Gaussian splatting presented an efficeint 3D representation methods that results in high quality and fast rendering speed. With the help of rasterization based rendering, Gaussian splatting bipassed the time consuming volumetric rendering process in NERFs for fast rendering times. However both these methods needs to be optimized in a cases by case basis. Another drawback of both of these methods is the need for a large number of views for high reconstruction quality. Feedforward methods has also been studied for 3D reconstruction, the goal being to allieviate the need for reconstructing in a scene by scene basis Recent works SRN, LFN, PixelSplat,MVSplat, GRM, LVSM have made substantial progress towards this regime.  Initial feedforward networks relied on utilizing camera poses and incorporated 3D priors for developing a generalizable 3D reconstruction method. Once trained, these methods need not be trained in a case by case basis for generalizing over unseen scenes. The first work to incorporate such a training regime utilized camera conditioning through $R,T$ matrices. Following works incorporated epilpolar constriants into the network for camera consistency and tend to perform better. Very recent works (Pixelsplat, MVSplat) utilized feedforward networks to model gaussain primitives. Specifically these works map sparse views to gaussian priomitives which can be later rasterized to synthesize novel views.




% As multi-view datasets are limited and expensive to collect, we looked towards synthetic data to curate a more diverse training set. In existing literature, synthetic data have been proposed several times as a way to increase the diversity and size of multiview datasets, as publicly available 3D scene data is limited and may be insufficient to train a highly generalizable NVS model. However, none of the previous methods using synthetic data have shown reconstruction quality surpassing those trained with real data. [Insert specific references and examples of models. Also, are we making this claim only for models trained 100\% on synthetic data or those that are a blend of real and synthetic data?]


% However, these models often exhibit limited cross-domain generalization, performing poorly on scenes that differ from their training data. [Insert evidence that these models lack cross-domain generalization] The lack of diversity in training domains likely contributes to this issue. Multi-view datasets are expensive to collect, and those used for training NVS models are limited and not diverse in the domains they represent. For instance, widely used scene-level datasets Re10k and ACID each include only a single category of scenes—living spaces and aerial shots, respectively. This highlights the limited diversity of available training datasets in terms of scene variety. [Insert more information backing our claim about datasets lacking diversity. Maybe also address object level? Maybe the size of these datasets? Maybe MVImgNet paper can have some references we can learn from]




% On the other hand, in the larger field of computer vision, large datasets and models that can scale with data and parameter size have shown to be very effective. [Insert specific CV models that benefited from a larger data size and parameter]. In particular, large computer vision models trained on a diverse training set show high generalizability to previously unseen domains. [Insert specific CV models that exhibit high generalizability from using diverse training set]. Keeping in mind that other computer vision models were able to learn cross-domain generalizability by training across a wide range of inputs through diverse and large datasets, we pose the question:


%  \newline
%  \newline
%  \textit{\textbf{Can we train a novel view synthesis model that generalizes better to unseen datasets by using a more diverse training dataset and an architecture that scales better with data? }}
% \newline
%  \newline
%  \newline
%  \textit{\textbf{Can we train a NVS model that scales with data and generalizes better to unseen datasets? }}
% \newline

% LVSM reconstructs a target view from sparse source views and their camera parameters represented by Plücker coordinates. During training, these source and target view tokens are combined and processed by a transformer block. The training objective focuses solely on reconstructing the target view, discarding the source tokens. However, our experiments revealed that this decoder-only design introduces a feature alignment issue: the target and source features become similar across all layers, as they share a feature space. Consequently, the transformer wastes computational resources modifying source tokens that are ultimately discarded, reducing efficiency. Additionally, this design makes LVSM vulnerable to noise or compression artifacts present in the source views. We also observed limited cross-domain performance when testing LVSM on datasets outside its training domain. This issue, while not unique to LVSM, stems from data scarcity in 3D vision. The combined size of all existing multiview 3D scene datasets is less than 100,000 scenes, significantly hindering performance on real-world scenarios outside the training distribution.






%  LVSM presents the first work for 3D inductive bias free NVS where a simple transformer model is trained to translate the target view plucker coordinates to the target views, conditioned with input views and the corresponding plucker coordinates. In addition LVSM uses additional training strategies like Q-K normalization that stabilizes the training process and a final sigmoid layer to lower the variance during the trianing process. We find that, this design although is effective in generalizing well to different methods has some inefficiencies which if addressed will improve the overall generation capability as well as the reconstruction quality. In this section we detail these problems and out approach towards solving it.



% The model is simply a decoder-only transformer which operates on source images, plucker coordinates that represent those source images, and plucker coordinates that represent a target camera. It directly produces a render from the target perspective. For the most part, LVSM uses a traditional transformer, in a similar fashion to a vision transformer. However, there are some notable differences – the paper describes a special initialization scheme, QK-normalization, and an additional sigmoid layer to lower variance during training.




% \subsection{Enhancing 3D generative models for 3D consistent generation}

% The use of diffusion models have been widely explored for generation of 3D scenes. Multiple works have been proposed in literature that adapts pretrained text-to-image models and pretrained image-to-video models for 3D consistent scene generation. Most of these works condition the diffusion model on camera parameters and learn the conditional distribution of multiple views given the camera poses. Given the chance to cherry pick and sample through the diffusion model multiple times, these models produce high quality results. However existing 3D scene generation models cannot mass produce synthetic data that can be used for finetuning substream models for high fidelity generation. Until now, no generalizable models  with high fidelity results have been proposed that can directly utilize the data generated by diffusion models.  We argue that this drawback is caused by a lack of analysis of the inference time generation process of diffusion models. Although extensive studies have been on performed on different training strategies for 3D consistent generation using diffusion models much less effort has been put into improving the inference time generation quality.


% Most 3D generative models for generation, generates N views of a scene each of dimension $(H \times W \times C)$ in parallel so that 3D consistency is preserved. The generation process starts with a random isotropic Gaussian noise of dimension $N \times H \times W \times C$ and undergoes a diffusion process of T steps which either converts it to a latent which is then decoded by a VAE decoder to produce multiview images. these multiview images are further used to 
% train a NERF or a Gaussian Splat, from where novel views of the scene can be generated. In the cases where the diffusion model generates high quality 3D consistent images this framework works perfectly. However in reality, diffusion models are sensitive to the sensitive to the input noise. Even for the simple case of Image generation, different noise inputs produce different qualiy results. Recent works have shed light on inference time scaling laws for generation where, the authors claim that the generation quality of diffusion models can be controlled by choosing the correct input noise with rejection sampling. Previous works have proposed similar claims for video generation models where the performance of video generation models drastically improved with improving the input noise schedule. To understand this consider this toy example. Suppose we want to generate an image (I1) using the diffusion model conditioned on a text prompt. starting with a gaussin noise N1, If we want to generate another image (I2) close to (I1), the desired noise is most likely closer to $N1$. Previous works have shown enhanced video generation results by choosing the starting noises across different frames close to each other. 
% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{ICCV2025-Author-Kit-Feb/figures/Ray-Transformer (21).pdf}
%     \vspace{-8mm}
%     \caption{\textbf{An illustration of our proposed transformer block} We utilize CAT3D, a multiview diffusion model to generate seven views conditioned on one view and its corresponding raymaps. Then we choose two random views form the generated views as the source views and the input conditioning view of the generative model to be the target of our large reconstruction network. Our large reconstruction model utilizes a special transformer block which we name Ray-Transformer. When real data is available, we utilize just the reconstruction transformer.}
%     \label{fig:my_label}
% \end{figure*}

% In our case. We use image to multi view variant of CAT3D as the base model for generating multiview images. For choosing the initial noise we follow a particular heuristic. Specifically, we make sure that the noises across different views are 3D consistent. Cat3D is a multiview diffusion model that generates 8 views simultaneously conditioned on the camera poses. Cat3D allows conditioning  on a particular view for generating the remaining views. Given the view to be conditioned, we choose a random noise for this view, lets call this V1 and the noise represented by N1 and corresponding rotation translation matrices denotes by $R_1,t_1$. For estimating the starting noise, we perform a warping operation on $N1$ denoted by 

% \begin{equation}
%     N_i = warp(N1, inv([Ri,ti])[R1,t1)]
% \end{equation}

% Where warp operation warps the coordinates of N1 to $N_i$. However we noticed that such a warping operation fails for cases which is outside of the scene. to handle for these cases at the same time to enhance consistency we marginally change the noise for such cases, specifically, for these cases we assign the noise as


% \begin{equation}
%     N_2 = \alpha N1+ (1-\alpha) \mathcal{N}(0,I)
% \end{equation}

% In short our effective starting noise is defined as 


% Although we use CAT3D, our method is generalizable across any 3D scene generation model

% Understanding the value synthetic data from generative models can bring, we propose a method to enhance diffusion based 3D generative models to produce high quality 3D consistent results. 



% One issue with LVSM’s architecture is that source features and target features are in the same intermediate latent space within the transformer. In other words, the same latent space represents the source features, which represent both the contents of the source images and their Plucker coordinates, and the target features, which represent the Plucker coordinates of the target (see \Cref{fig:src_lvsm_pca} for more details). In addition, the tokens that are produced by the final transformer block which represent the source features are ultimately discarded. This suggests that the transformer is wasting capacity keeping the source and target features aligned in a single space. We believe that this behavior happens because the transformer cannot differentiate between the source and target tokens during optimization. To fix this, we make the transformer blocks aware of the difference between source and target tokens tokens using style modulation. \textcolor{red}{Style modulation is often used in GANs to ….}



% Specifically, we signify the source and target tokens using specialized embeddings and infuse them with scale and shift operation. We call the corresponding transformer block (Reconstruct Any)ray-transformer. 


% To this end we propose a simple and effective scheme using our disentangled transformer 

% For object level synthesis, we follow GS-LRM and LVSM and we train on Objaverse dataset and test on 
% GSO, ABO datasets. Additionally we also test on DTU dataset for objects. For object level training, we use 4 input view and 8 target views. On contrast to LVSM that uses a batchsize of 64, because of resource constraints, we train using a batch size of 32. The training for the scene experiments takes a total of 2 days and for objects take a total of 4 days.



%  \subsection{synthetic data size vs performance}
%  \subsection{PCA visualziation for our network}


